Benchmark Assessment for DeepSpeed Optimization Library

Deep Learning (DL) models are widely used in machine learning due to their performance and ability to deal with large datasets while producing high accuracy and performance metrics. The size of such datasets and the complexity of DL models cause such models to be complex, consuming large amount of resources and time to train. Many recent libraries and applications are introduced to deal with DL complexity and efficiency issues. In this paper, we evaluated one example, Microsoft DeepSpeed library through classification tasks. DeepSpeed public sources reported classification performance metrics on the LeNet architecture. We extended this through evaluating the library on several modern neural network architectures, including convolutional neural networks (CNNs) and Vision Transformer (ViT). Results indicated that DeepSpeed, while can make improvements in some of those cases, it has no or negative impact on others.

==> Benchmark Assessment for DeepSpeed Optimization Library/unused_figures.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall.png}
    \caption{Overall Performs (DS: Adam+CYCLICLR, Normal: SGD) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall_sgd_cycliclr.png}
    \caption{Overall Performs (SGD + CYCLICLR) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall_adam_cycliclr.png}
    \caption{Overall Performs (Adam + CYCLICLR) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/lenet.png}
      \caption{LeNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/alexnet.png}
      \caption{AlexNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/vgg.png}
      \caption{VGG}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/squeezenet.png}
      \caption{SqueezeNet}
    \end{subfigure}
    
    \caption{\gbl{Figure needs to be redraw}}
    \label{fig:clustering}
\end{figure}


\begin{figure}[!tb]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/resnet.png}
      \caption{ResNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/densenet.png}
      \caption{DenseNet}
    \end{subfigure}
    
    \caption{\gbl{Figure needs to be redraw}}
    \label{fig:clustering}
\end{figure}

==> unused_figures.tex <==
\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall.png}
    \caption{Overall Performs (DS: Adam+CYCLICLR, Normal: SGD) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall_sgd_cycliclr.png}
    \caption{Overall Performs (SGD + CYCLICLR) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \includegraphics[width=.95\textwidth]{figures/overall_adam_cycliclr.png}
    \caption{Overall Performs (Adam + CYCLICLR) \gbl{Figure needs to be redraw}}
    \label{fig:overall}
\end{figure}

\begin{figure}[!tb]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/lenet.png}
      \caption{LeNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/alexnet.png}
      \caption{AlexNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/vgg.png}
      \caption{VGG}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/squeezenet.png}
      \caption{SqueezeNet}
    \end{subfigure}
    
    \caption{\gbl{Figure needs to be redraw}}
    \label{fig:clustering}
\end{figure}


\begin{figure}[!tb]
    \centering
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/resnet.png}
      \caption{ResNet}
    \end{subfigure}
    
    \begin{subfigure}[b]{1.0\textwidth}
      \centering
      \includegraphics[width=.95\textwidth]{figures/densenet.png}
      \caption{DenseNet}
    \end{subfigure}
    
    \caption{\gbl{Figure needs to be redraw}}
    \label{fig:clustering}
\end{figure}
